Choice of the Parameters in A Primal-Dual Algorithm for Bregman Iterated Variational Regularization

Focus of this work is solving a non-smooth constraint minimization problem by a primal-dual splitting algorithm involving proximity operators. The problem is penalized by the Bregman divergence associated with the non-smooth total variation (TV) functional. We analyse two aspects: Firstly, the convergence of the regularized solution of the minimization problem to the minimum norm solution. Second, the convergence of the iteratively regularized minimizer to the minimum norm solution by a primal-dual algorithm. For both aspects, we use the assumption of a variational source condition (VSC). This work emphasizes the impact of the choice of the parameters in stabilization of a primal-dual algorithm. Rates of convergence are obtained in terms of some concave, positive definite index function. The algorithm is applied to a simple two dimensional image processing problem. Sufficient error analysis profiles are provided based on the size of the forward operator and the noise level in the measurement.

==> iopart10.clo.tex <==
%% 
%% This is file `iopart10.clo'
%% 
%% This file is distributed in the hope that it will be useful, 
%% but WITHOUT ANY WARRANTY; without even the implied warranty of 
%% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE. 
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\ProvidesFile{iopart10.clo}[1997/01/13 v1.0 IOP Book file (size option)]
\renewcommand\normalsize{%
   \@setfontsize\normalsize\@xpt\@xiipt
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\newcommand\small{%
   \@setfontsize\small\@ixpt{11}%
   \abovedisplayskip 8.5\p@ \@plus3\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus2\p@
   \belowdisplayshortskip 4\p@ \@plus2\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 4\p@ \@plus2\p@ \@minus2\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand\footnotesize{%
   \@setfontsize\footnotesize\@viiipt{9.5}%
   \abovedisplayskip 6\p@ \@plus2\p@ \@minus4\p@
   \abovedisplayshortskip \z@ \@plus\p@
   \belowdisplayshortskip 3\p@ \@plus\p@ \@minus2\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 3\p@ \@plus\p@ \@minus\p@
               \parsep 2\p@ \@plus\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand\scriptsize{\@setfontsize\scriptsize\@viipt\@viiipt}
\newcommand\tiny{\@setfontsize\tiny\@vpt\@vipt}
\newcommand\large{\@setfontsize\large\@xiipt{14}}
\newcommand\Large{\@setfontsize\Large\@xivpt{18}}
\newcommand\LARGE{\@setfontsize\LARGE\@xviipt{22}}
\newcommand\huge{\@setfontsize\huge\@xxpt{25}}
\newcommand\Huge{\@setfontsize\Huge\@xxvpt{30}}
\if@twocolumn
  \setlength\parindent{12\p@}
\else
  \setlength\parindent{15\p@}
\fi
\setlength\headheight{12\p@}
\setlength\headsep   {12\p@}
\setlength\topskip   {10\p@}
\setlength\footskip{20\p@}
\setlength\maxdepth{.5\topskip}
\setlength\@maxdepth\maxdepth
\setlength\textwidth{31pc}
\setlength\textheight{49pc}
\setlength\oddsidemargin  {24\p@}
\setlength\evensidemargin {24\p@}
\setlength\marginparwidth {72\p@}
\setlength\marginparsep {10\p@}
\setlength\marginparpush{5\p@}
\setlength\topmargin{\z@}
\setlength\footnotesep{6.65\p@}
\setlength{\skip\footins}  {9\p@ \@plus 4\p@ \@minus 2\p@}
\setlength\floatsep       {12\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\textfloatsep   {20\p@ \@plus 2\p@ \@minus 4\p@}
\setlength\intextsep      {12\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\dblfloatsep    {12\p@ \@plus 2\p@ \@minus 2\p@}
\setlength\dbltextfloatsep{20\p@ \@plus 2\p@ \@minus 4\p@}
\setlength\@fptop{0\p@}
\setlength\@fpsep{8\p@ \@plus 2fil}
\setlength\@fpbot{0\p@}
\setlength\@dblfptop{0\p@}
\setlength\@dblfpsep{8\p@ \@plus 2fil}
\setlength\@dblfpbot{0\p@}
\setlength\partopsep{2\p@ \@plus 1\p@ \@minus 1\p@}
\def\@listI{\leftmargin\leftmargini
            \parsep=\z@ 
            \topsep=5\p@ \@plus3\p@ \@minus3\p@
            \itemsep=3\p@ \@plus2\p@ \@minus\p@}
\let\@listi\@listI
\@listi
\def\@listii {\leftmargin\leftmarginii
     \labelwidth\leftmarginii
     \advance\labelwidth-\labelsep
     \topsep=2\p@ \@plus2\p@ \@minus\p@
     \parsep=\z@
     \itemsep=\parsep}
\def\@listiii{\leftmargin\leftmarginiii
     \labelwidth\leftmarginiii
     \advance\labelwidth-\labelsep
     \topsep=\z@
     \parsep=\z@
     \partopsep=\z@
     \itemsep=\z@}
\def\@listiv {\leftmargin\leftmarginiv
     \labelwidth\leftmarginiv
     \advance\labelwidth-\labelsep}
\def\@listv  {\leftmargin\leftmarginv
     \labelwidth\leftmarginv
     \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
     \labelwidth\leftmarginvi
     \advance\labelwidth-\labelsep}
\endinput
%% 
%% End of file `iopart.clo'.



==> iopart12.clo.tex <==
%% 
%% This is file `iopart12.clo'
%% 
%% This file is distributed in the hope that it will be useful, 
%% but WITHOUT ANY WARRANTY; without even the implied warranty of 
%% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE. 
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
\ProvidesFile{iopart12.clo}[1997/01/15 v1.0 LaTeX2e file (size option)]
\renewcommand\normalsize{%
   \@setfontsize\normalsize\@xiipt{16}%
   \abovedisplayskip 12\p@ \@plus3\p@ \@minus7\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6.5\p@ \@plus3.5\p@ \@minus3\p@
   \belowdisplayskip \abovedisplayskip
   \let\@listi\@listI}
\normalsize
\newcommand\small{%
   \@setfontsize\small\@xipt{14}%
   \abovedisplayskip 11\p@ \@plus3\p@ \@minus6\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6.5\p@ \@plus3.5\p@ \@minus3\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 9\p@ \@plus3\p@ \@minus5\p@
               \parsep 4.5\p@ \@plus2\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand\footnotesize{%
%   \@setfontsize\footnotesize\@xpt\@xiipt
   \@setfontsize\footnotesize\@xpt{13}%
   \abovedisplayskip 10\p@ \@plus2\p@ \@minus5\p@
   \abovedisplayshortskip \z@ \@plus3\p@
   \belowdisplayshortskip 6\p@ \@plus3\p@ \@minus3\p@
   \def\@listi{\leftmargin\leftmargini
               \topsep 6\p@ \@plus2\p@ \@minus2\p@
               \parsep 3\p@ \@plus2\p@ \@minus\p@
               \itemsep \parsep}%
   \belowdisplayskip \abovedisplayskip
}
\newcommand\scriptsize{\@setfontsize\scriptsize\@viiipt{9.5}}
\newcommand\tiny{\@setfontsize\tiny\@vipt\@viipt}
\newcommand\large{\@setfontsize\large\@xivpt{18}}
\newcommand\Large{\@setfontsize\Large\@xviipt{22}}
\newcommand\LARGE{\@setfontsize\LARGE\@xxpt{25}}
\newcommand\huge{\@setfontsize\huge\@xxvpt{30}}
\let\Huge=\huge
\if@twocolumn
  \setlength\parindent{14\p@}
\else
  \setlength\parindent{18\p@}
\fi
\setlength\headheight{14\p@}
\setlength\headsep{14\p@}
\setlength\topskip{12\p@}
\setlength\footskip{24\p@}
\setlength\maxdepth{.5\topskip}
\setlength\@maxdepth\maxdepth
\setlength\textwidth{37.2pc}
\setlength\textheight{56pc}
\setlength\oddsidemargin  {\z@}
\setlength\evensidemargin {\z@}
\setlength\marginparwidth {72\p@}
\setlength\marginparsep{10\p@}
\setlength\marginparpush{5\p@}
\setlength\topmargin{-12pt}
\setlength\footnotesep{8.4\p@}
\setlength{\skip\footins} {10.8\p@ \@plus 4\p@ \@minus 2\p@}
\setlength\floatsep       {14\p@ \@plus 2\p@ \@minus 4\p@}
\setlength\textfloatsep   {24\p@ \@plus 2\p@ \@minus 4\p@}
\setlength\intextsep      {16\p@ \@plus 4\p@ \@minus 4\p@}
\setlength\dblfloatsep    {16\p@ \@plus 2\p@ \@minus 4\p@}
\setlength\dbltextfloatsep{24\p@ \@plus 2\p@ \@minus 4\p@}
\setlength\@fptop{0\p@}
\setlength\@fpsep{10\p@ \@plus 1fil}
\setlength\@fpbot{0\p@}
\setlength\@dblfptop{0\p@}
\setlength\@dblfpsep{10\p@ \@plus 1fil}
\setlength\@dblfpbot{0\p@}
\setlength\partopsep{3\p@ \@plus 2\p@ \@minus 2\p@}
\def\@listI{\leftmargin\leftmargini
     \parsep=\z@
     \topsep=6\p@  \@plus3\p@ \@minus3\p@
     \itemsep=3\p@ \@plus2\p@ \@minus1\p@}
\let\@listi\@listI
\@listi
\def\@listii {\leftmargin\leftmarginii
     \labelwidth\leftmarginii
     \advance\labelwidth-\labelsep
     \topsep=3\p@ \@plus2\p@ \@minus\p@
     \parsep=\z@
     \itemsep=\parsep}
\def\@listiii{\leftmargin\leftmarginiii
     \labelwidth\leftmarginiii
     \advance\labelwidth-\labelsep
     \topsep=\z@
     \parsep=\z@
     \partopsep=\z@
     \itemsep=\z@}
\def\@listiv {\leftmargin\leftmarginiv
     \labelwidth\leftmarginiv
     \advance\labelwidth-\labelsep}
\def\@listv{\leftmargin\leftmarginv
     \labelwidth\leftmarginv
     \advance\labelwidth-\labelsep}
\def\@listvi {\leftmargin\leftmarginvi
     \labelwidth\leftmarginvi
     \advance\labelwidth-\labelsep}
\endinput
%% 
%% End of file `iopart12.clo'.



==> mysty.tex <==
%======================================================
% 1. page format
%======================================================

% \oddsidemargin1cm
% \evensidemargin1cm
% \topmargin1cm
% \headheight0.3cm
% \headsep1cm
% \textheight20cm
% \footskip1cm
% \textwidth14cm
% \marginparwidth2.5cm

%======================================================
% 2. packages and classes
%======================================================

%\usepackage[pdftex]{hyperref} 
% \usepackage[pdfpagelabels]{hyperref} 
% \hypersetup{colorlinks=true,
% linkcolor=blue,
% citecolor=blue,
% plainpages=false}
% \usepackage{todonotes}
% %\usepackage[notref]{showkeys}    
% \usepackage{amssymb}
% %\usepackage{german}
% % \usepackage{latexsym}
% \usepackage{amsmath}
% \usepackage{amsthm}
% \usepackage{amsfonts}
% \usepackage{epsfig}
% \usepackage{pb-diagram}         % Diagramme!
% \usepackage{colordvi,cite}
% \usepackage{color}
% \definecolor{labelkey}{gray}{.75}
% \usepackage[ignoreunlbld,ignoreunlbld,nomsgs]{refcheck}
% %\usepackage[noeepic]{qtree}  		% B�ume!
% %\usepackage{psfrag}
% %\usepackage{amsxtra}
% %\usepackage{hhline}
% \usepackage{nccmath}
% 
% \usepackage{makeidx}
% \usepackage{placeins}
% \usepackage{showkeys}
% \usepackage{datetime}
% \ddmmyyyydate % format date to 8/3/09
% %\usepackage{verbatim}
% \usepackage{xkeyval}
% \usepackage{fancyvrb}
% \input xstring
% %\usepackage[T1]{fontenc}
% \usepackage{graphicx}

% HYPERREF Package defines Hyperlinks within the PDF Document
% this works only with PDF, so please remove block comment before
% processing PdfLaTeX!
%
%\usepackage[pdftex]{hyperref}
%\hypersetup{
%    bookmarks=true,         % show bookmarks bar?
%    unicode=false,          % non-Latin characters in Acrobat�s bookmarks
%    pdftoolbar=true,        % show Acrobat�s toolbar?
%    pdfmenubar=true,        % show Acrobat�s menu?
%    pdffitwindow=true,      % page fit to window when opened
%    pdftitle={Inverse Modelling},    % title
%    pdfauthor={Nakamura and Potthast},     % author
%    pdfsubject={Inverse Problems, Paramter Estimation, Data Assimilation},   %
%    pdfnewwindow=true,      % links in new window
%    pdfkeywords={}, % list of keywords
%    colorlinks=true,       % false: boxed links; true: colored links
%    linkcolor=red,          % color of internal links
%    citecolor=green,        % color of links to bibliography
%    filecolor=magenta,      % color of file links
%    urlcolor=cyan           % color of external links
%}

%======================================================
% 3. index at the end of the document
%======================================================

\makeindex

%======================================================
% 4. caligraphic abbreviations
%======================================================

% small letters
% \cal a,b,... give special characters!

% large letters
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}
\newcommand{\cm}{{\mathcal m}}

%======================================================
% 5. tilde abbreviations
%======================================================

% tilde small letters

\newcommand{\ta}{\tilde{a}}
\newcommand{\tb}{\tilde{b}}
\newcommand{\tc}{\tilde{c}}
\newcommand{\td}{\tilde{d}}
\newcommand{\te}{\tilde{e}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tg}{\tilde{g}}
\newcommand{\tih}{\tilde{h}}
\newcommand{\ti}{\tilde{i}}
\newcommand{\tj}{\tilde{j}}
\newcommand{\tk}{\tilde{k}}
\newcommand{\tl}{\tilde{l}}
\newcommand{\tm}{\tilde{m}}
\newcommand{\tn}{\tilde{n}}
\newcommand{\tio}{\tilde{o}}
\newcommand{\tp}{\tilde{p}}
\newcommand{\tq}{\tilde{q}}
%\newcommand{\tr}{\tilde{r}}
\newcommand{\ts}{\tilde{s}}
\newcommand{\tit}{\tilde{t}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tv}{\tilde{v}}
\newcommand{\tw}{\tilde{w}}
\newcommand{\tx}{\tilde{x}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tz}{\tilde{z}}

% tilde large letters

\newcommand{\tA}{\tilde{A}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tC}{\tilde{C}}
\newcommand{\tD}{\tilde{D}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\tH}{\tilde{H}}
\newcommand{\tI}{\tilde{I}}
\newcommand{\tJ}{\tilde{J}}
\newcommand{\tK}{\tilde{K}}
\newcommand{\tL}{\tilde{L}}
\newcommand{\tM}{\tilde{M}}
\newcommand{\tN}{\tilde{N}}
\newcommand{\tO}{\tilde{O}}
\newcommand{\tP}{\tilde{P}}
\newcommand{\tQ}{\tilde{Q}}
\newcommand{\tR}{\tilde{R}}
\newcommand{\tS}{\tilde{S}}
\newcommand{\tT}{\tilde{T}}
\newcommand{\tU}{\tilde{U}}
\newcommand{\tV}{\tilde{V}}
\newcommand{\tW}{\tilde{W}}
\newcommand{\tX}{\tilde{X}}
\newcommand{\tY}{\tilde{Y}}
\newcommand{\tZ}{\tilde{Z}}

% tilde small greec letters

\newcommand{\talpha}{\tilde{\alpha}}
\newcommand{\tbeta}{\tilde{\beta}}
\newcommand{\tgamma}{\tilde{\gamma}}
\newcommand{\tdelta}{\tilde{\delta}}
\newcommand{\tepsilon}{\tilde{\epsilon}}
\newcommand{\tzeta}{\tilde{\zeta}}
\newcommand{\teta}{\tilde{\eta}}
\newcommand{\ttheta}{\tilde{\theta}}
\newcommand{\tiota}{\tilde{\iota}}
\newcommand{\tkappa}{\tilde{\kappa}}
\newcommand{\tlambda}{\tilde{\lambda}}
\newcommand{\tmu}{\tilde{\mu}}
\newcommand{\tnu}{\tilde{\nu}}
\newcommand{\txi}{\tilde{\xi}}
%\newcommand{\tomicron}{\tilde{\omicron}}
\newcommand{\tpi}{\tilde{\pi}}
\newcommand{\trho}{\tilde{\rho}}
\newcommand{\tsigma}{\tilde{\sigma}}
\newcommand{\ttau}{\tilde{\tau}}
\newcommand{\tupsilon}{\tilde{\upsilon}}
\newcommand{\tpsi}{\tilde{\psi}}
\newcommand{\tvarphi}{\tilde{\varphi}}
\newcommand{\tomega}{\tilde{\omega}}

% tilde large greec letters

\newcommand{\tGamma}{\tilde{\Gamma}}
\newcommand{\tDelta}{\tilde{\Delta}}
\newcommand{\tTheta}{\tilde{\Theta}}
\newcommand{\tLambda}{\tilde{\Lambda}}
\newcommand{\tXi}{\tilde{\Xi}}
\newcommand{\tPi}{\tilde{\Pi}}
\newcommand{\tSigma}{\tilde{\Sigma}}
\newcommand{\tPsi}{\tilde{\Psi}}
\newcommand{\tOmega}{\tilde{\Omega}}

%======================================================
% 6. hat abbreviations
%======================================================

% hat small letters

\newcommand{\ha}{\hat{a}}
\newcommand{\hb}{\hat{b}}
\newcommand{\hc}{\hat{c}}
\newcommand{\hd}{\hat{d}}
\newcommand{\he}{\hat{e}}
\newcommand{\hf}{\hat{f}}
\newcommand{\hg}{\hat{g}}
\newcommand{\hh}{\hat{h}}
\newcommand{\hi}{\hat{i}}
\newcommand{\hj}{\hat{j}}
\newcommand{\hk}{\hat{k}}
\newcommand{\hl}{\hat{l}}
\newcommand{\hm}{\hat{m}}
\newcommand{\hn}{\hat{n}}
\newcommand{\ho}{\hat{o}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hr}{\hat{r}}
\newcommand{\hs}{\hat{s}}
\newcommand{\hatt}{\hat{t}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}

% hat large letters

\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hI}{\hat{I}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hM}{\hat{M}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hO}{\hat{O}}
\newcommand{\hP}{\hat{P}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hR}{\hat{R}}
\newcommand{\hS}{\hat{S}}
\newcommand{\hT}{\hat{T}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hW}{\hat{W}}
\newcommand{\hX}{\hat{X}}
\newcommand{\hY}{\hat{Y}}
\newcommand{\hZ}{\hat{Z}}

% hat greec letters

\newcommand{\halpha}{\hat{\alpha}}
\newcommand{\hbeta}{\hat{\beta}}
\newcommand{\hgamma}{\hat{\gamma}}
\newcommand{\hdelta}{\hat{\delta}}
\newcommand{\hepsilon}{\hat{\epsilon}}
\newcommand{\hzeta}{\hat{\zeta}}
\newcommand{\heta}{\hat{\eta}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\hiota}{\hat{\iota}}
\newcommand{\hkappa}{\hat{\kappa}}
\newcommand{\hlambda}{\hat{\lambda}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\hnu}{\hat{\nu}}
\newcommand{\hxi}{\hat{\xi}}
%\newcommand{\homicron}{\hat{\omicron}}
\newcommand{\hpi}{\hat{\pi}}
\newcommand{\hrho}{\hat{\rho}}
\newcommand{\hsigma}{\hat{\sigma}}
\newcommand{\htau}{\hat{\tau}}
\newcommand{\hupsilon}{\hat{\upsilon}}
\newcommand{\hpsi}{\hat{\psi}}
\newcommand{\homega}{\hat{\omega}}

% hat caligraphic letters

\newcommand{\hGamma}{\hat{\gamma}}
\newcommand{\hDelta}{\hat{\Delta}}
\newcommand{\hTheta}{\hat{\Theta}}
\newcommand{\hLambda}{\hat{\Lambda}}
\newcommand{\hXi}{\hat{\Xi}}
\newcommand{\hPi}{\hat{\Pi}}
\newcommand{\hSigma}{\hat{\Sigma}}
\newcommand{\hPsi}{\hat{\Psi}}
\newcommand{\hOmega}{\hat{\Omega}}


%======================================================
% 7. bold abbreviations
%======================================================

% bold small letters

%\newcommand{\ba}{{\bf a}}
%\newcommand{\bb}{{\bf b}}
%\newcommand{\bc}{{\bf c}}
%\newcommand{\bd}{{\bf d}}
%\newcommand{\be}{{\bf e}}
\newcommand{\boldf}{{\bf f}}
\newcommand{\bg}{{\bf g}}
\newcommand{\bh}{{\bf h}}
%\newcommand{\bi}{{\bf i}}
\newcommand{\bj}{{\bf j}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bl}{{\bf l}}
\newcommand{\bm}{{\bf m}}
\newcommand{\bn}{{\bf n}}
\newcommand{\bo}{{\bf o}}
\newcommand{\bp}{{\bf p}}
\newcommand{\bq}{{\bf q}}
%\newcommand{\br}{{\bf r}}
%\newcommand{\bs}{{\bf s}}
\newcommand{\bt}{{\bf t}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bz}{{\bf z}}

% bold large letters

\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bG}{{\bf G}}
\newcommand{\bH}{{\bf H}}
\newcommand{\btH}{{\bf \tilde{H}}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bJ}{{\bf J}}
\newcommand{\bK}{{\bf K}}
\newcommand{\btK}{{\bf \tilde{K}}}
\newcommand{\bL}{{\bf L}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bO}{{\bf O}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bQ}{{\bf Q}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\btS}{{\bf \tilde{S}}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bW}{{\bf W}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bZ}{{\bf Z}}

% bold greec letters
% \newcommand{\}{\mbox{\boldmath{$\alpha$}}}
%\newcommand{\bbeta}{\mbox{\boldmath{$\beta$}}}
% \newcommand{\bchi}{\mbox{\boldmath{$\chi$}}}
% \newcommand{\bgamma}{\mbox{\boldmath{$\gamma$}}}
% \newcommand{\bdelta}{\mbox{\boldmath{$\delta$}}}
% \newcommand{\bepsilon}{\mbox{\boldmath{$\epsilon$}}}
% \newcommand{\bzeta}{\mbox{\boldmath{$\zeta$}}}
% \newcommand{\boldeta}{\mbox{\boldmath{$\eta$}}}
% \newcommand{\btheta}{\mbox{\boldmath{$\theta$}}}
% \newcommand{\biota}{\mbox{\boldmath{$\iota$}}}
% \newcommand{\bkappa}{\mbox{\boldmath{$\kappa$}}}
% \newcommand{\blambda}{\mbox{\boldmath{$\lambda$}}}
% \newcommand{\bmu}{\mbox{\boldmath{$\mu$}}}
% \newcommand{\bnu}{\mbox{\boldmath{$\nu$}}}
% \newcommand{\bxi}{\mbox{\boldmath{$\xi$}}}
% \newcommand{\bomicron}{\mbox{\boldmath{$\omicron$}}}
% \newcommand{\bpi}{\mbox{\boldmath{$\pi$}}}
% \newcommand{\brho}{\mbox{\boldmath{$\rho$}}}
% \newcommand{\bsigma}{\mbox{\boldmath{$\sigma$}}}
% \newcommand{\btau}{\mbox{\boldmath{$\tau$}}}
% \newcommand{\bupsilon}{\mbox{\boldmath{$\upsilon$}}}
% \newcommand{\bpsi}{\mbox{\boldmath{$\psi$}}}
% \newcommand{\bomega}{\mbox{\boldmath{$\omega$}}}
% \newcommand{\bvarphi}{\mbox{\boldmath{$\varphi$}}}
% \newcommand{\tbvarphi}{\mbox{\boldmath{$\tilde{\varphi}$}}}

% bold large Greec letters

% 

% bold caligraphic letters

% ? \newcommand{\bcM}{\mbox{\boldmath $\cM$}}
% ? \newcommand{\bsM}{\mbox{\boldmath $\scriptstyle M$}}


%======================================================
% 8. ast abbreviations
%======================================================

% ast small letters


% ast large letters

\newcommand{\Aast}{A^{\ast}}
\newcommand{\Fast}{F^{\ast}}
\newcommand{\Gast}{G^{\ast}}
\newcommand{\Kast}{K^{\ast}}
\newcommand{\Sast}{S^{\ast}}

% ast greek letters

% ast caligraphic letters

\newcommand{\cFast}{{\mathcal F}^{\ast}}

%======================================================
% 10. basic mathematics abbreviations
%======================================================

%======================================================
% 11. special functional analysis
%======================================================

\newcommand{\fd}{f^{(\delta)}}
\newcommand{\varphid}{\varphi^{(\delta)}}

%======================================================
% 12. special acoustic scattering 
%======================================================


%======================================================
% 18. special miscellaneous
%======================================================

% time derivatives
\newcommand{\ddt}[1]{\stackrel{{\bf .}}{#1}}
\newcommand{\Dp}{\stackrel{{\bf .}}{D}}
\newcommand{\Bp}{\stackrel{{\bf .}}{B}}

% demand
\newcommand{\demand}{\stackrel{!}{=}}
\newcommand{\argmax}{{\rm argmax} }

\newcommand{\dir}{\mbox{dir}\,}
\newcommand{\bset}[2]{\left\{#1\,\left|\,#2\right.\right\}}
\newcommand{\map}[3]{#1:\,#2\rightarrow #3\,}
\newcommand{\mmap}[3]{#1:\,#2\rightrightarrows #3\,}
\newcommand{\sph}{\set{S}}
%\newcommand{\qed}{\hfill $\Box$ \\ \medskip}

\newcommand{\LXY}{{\mathcal L}(X,Y)}
\newcommand{\LX}{{\mathcal L}(X)}
\newcommand{\ra}{{\mathcal R}(A)}
\newcommand{\rad}{{\mathcal R}(A^{\dagger})}
\newcommand{\ras}{{\mathcal R}(A^{*})}
\newcommand{\ora}{\overline{{\mathcal R}(A)}}

\newcommand{\Di}{D_{i}}
\newcommand{\Dast}{D_{\ast}}
\newcommand{\Had}{H^{\ast}}
\newcommand{\Sad}{S^{\ast}}
\newcommand{\uinfast}{u^{\infty}_{\ast}}
\newcommand{\uinfm}{u^{\infty}_{\delta}}
\newcommand{\usast}{u^{s}_{\ast}}
\newcommand{\uast}{u_{\ast}}
\newcommand{\ualpha}{u_{\alpha}}
\newcommand{\uinf}{u^{\infty}}
\newcommand{\us}{u^{s}}
\newcommand{\ui}{u^{i}}
\newcommand{\rast}{r_{\ast}}
\newcommand{\rastperp}{r_{\ast \perp}}
\newcommand{\rdelta}{r_{\delta}}
\newcommand{\udelta}{u_{\delta}}
\newcommand{\udeltainf}{u_{\delta}^{\infty}}
\newcommand{\vgs}{v^{s}_{g}}
\newcommand{\vg}{v_{g}}
\newcommand{\vgz}{v_{g(\cdot,z)}}
\newcommand{\vtgz}{v_{\tg(\cdot,z)}}
\newcommand{\vginf}{v^{\infty}_{g}}
\newcommand{\vtginf}{v^{\infty}_{\tg(\cdot,z)}}
\newcommand{\sdf}{{\mathcal S}}
\newcommand{\FF}{{\mathcal F}}
\newcommand{\Chi}{{\mathcal X}}
\newcommand{\Chil}{{\mathcal X}_\Lambda}
\newcommand{\Chinl}{{\mathcal X}_{-\Lambda}}
\newcommand{\uinfk}{u^{\infty}_m}
\newcommand{\usk}{u^{s}_m}
\newcommand{\uik}{u^{i}_m}
\newcommand{\psikl}{\psi_{(k,l)}}
\newcommand{\cMkl}{\cM_{\mij}}
\newcommand{\psikh}{\widehat{\psi}_m}
\newcommand{\apd}{\Omega_a}
\newcommand{\apdb}{\Omega_b}
\newcommand{\apdcl}{\overline{\Omega}_a}
\newcommand{\apdclb}{\overline{\Omega}_b}
\newcommand{\apdo}{\Omega_{0}}
\newcommand{\apdocl}{\overline{\Omega}_{0}}
\newcommand{\apdz}{\Omega_{z}}
\newcommand{\ffsurf}{R\set{S} }
\newcommand{\ffd}{\set{S}}
\newcommand{\ffdl}{-\Lambda}
\newcommand{\ffo}{F}
\newcommand{\ffol}{F}
\newcommand{\slo}{\mathcal{S}}
\newcommand{\hwf}{H}
\newcommand{\tslo}{\mathcal{W}}
\newcommand{\sslo}{\mathcal{W}^s}
\newcommand{\scd}{\Omega}
\newcommand{\scdcl}{\overline{\Omega}}
\newcommand{\exter}{\rem\!\setminus\!\scdcl}
\newcommand{\extercl}{\rem\!\setminus\!\scd}
\newcommand{\exterapd}{\rem\!\setminus\!\apdcl}
\newcommand{\exterapdcl}{\rem\!\setminus\!\apd}
\newcommand{\ild}{\set{E}}
\newcommand{\recdom}{\set{Q}}
\newcommand{\uff}{u^{\infty}}
\newcommand{\vff}{v^{\infty}}
\newcommand{\wff}{w^{\infty}}
\newcommand{\ffps}{ \Phi^\infty }
\newcommand{\bvff}{{\mathcal B}}
\newcommand{\tbvff}{\widetilde{{\mathcal B}}}
\newcommand{\rev}{{\mathcal R}}
\newcommand{\bpo}{{\mathcal A}}
\newcommand{\bpoa}{{\mathcal A}_\alpha}
\newcommand{\bdy}[1]{\partial{#1}}
\newcommand{\gps}{g_*}
\newcommand{\gal}{g_{\alpha}}
\newcommand{\galo}{g_{\alpha}}
\newcommand{\usrec}{u^{s}_\alpha}
\newcommand{\urec}{u_\alpha}
\newcommand{\mi}{{\boldsymbol n}}
\newcommand{\mij}{{\boldsymbol j}}
\newcommand{\ind}{\cN}
\newcommand{\indj}{\cJ}

%======================================================
% mathematical abbreviations: sets, norms, scalar
% products etc.  
%======================================================

\newcommand{\Complex}{\mathbb{C}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\M}{\mathbb{M}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\L}{\mathbb{L}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Zo}{\mathbb{Z}\setminus\{0\}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\mZ}{\mathbb{Z}}
\newcommand{\mS}{\mathbb{S}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\betr}[1]{|#1|}
%\newcommand{\mod}[1]{|#1|}
\newcommand{\Bbetr}[1]{\Big|#1\Big|}
\newcommand{\Lbetr}[1]{\left|#1\right|}
\newcommand{\curl}{{\rm curl \;}}
\newcommand{\dist}{{\rm dist \;}}

\newcommand{\tte}{\begin{flushright}$\Box$\end{flushright}}
\newcommand{\menge}[1]{\mbox{$\left\{ #1 \right\} $}}
\newcommand{\set}[1]{\mbox{$\left\{ #1 \right\} $}}
\newcommand{\Bmenge}[1]{\Big\{ #1 \Big\}}
\newcommand{\czz}{}
\newcommand{\norm}[1]{|| #1||}
\newcommand{\Bnorm}[1]{\Big|\Big| #1\Big|\Big|}  
\newcommand{\Lnorm}[1]{\left|\left| #1\right|\right|}  
\newcommand{\scal}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\Bscal}[2]{\Big\langle #1 , #2 \Big\rangle}
\renewcommand{\Im}{{\rm Im}}
\renewcommand{\Re}{{\rm Re}}
\newcommand{\Ind}{{\rm Ind \;}}
\newcommand{\cone}{{\rm co}}
\newcommand{\grad}{{\rm grad \;}}
\newcommand{\Grad}{{\rm Grad \;}}
\newcommand{\rmmod}{{\rm \; mod \;}}
\renewcommand{\div}{{\rm div \;}}
\newcommand{\Div}{{\rm Div \;}}
\newcommand{\FT}{{\mathcal FT}}
\newcommand{\diag}[1]{{\rm diag}\left\{ #1 \right\}}
\newcommand{\spart}[1]{{\rm spart}\left\{ #1 \right\}}
\newcommand{\myarr}[1]{\left( \begin{array}{cccccccccccccccccc}#1\end{array}\right)}

%\newcommand{\for}{\mbox{ for }}
\newcommand{\ow}{\mbox{ otherwise }}
\newcommand{\supp}{{\rm supp }} 
\newcommand{\kernel}{\mbox{null}\,}
\newcommand{\im}{{i}} 
\newcommand{\re}{\mathbb{R}}
\newcommand{\rep}{\mathbb{R}_+}
\newcommand{\ret}{\mathbb{R}^2}
\newcommand{\ren}{\mathbb{R}^n}
\newcommand{\rem}{\mathbb{R}^m}
\newcommand{\rg}{\mathbb{R}^{N_1}\times \mathbb{R}^{N_2}}
\newcommand{\rgp}{\rep^{N_1}\times \rep^{N_2}}
\newcommand{\kg}{\mathbb{K}^{N_1}\times \mathbb{K}^{N_2}}
\newcommand{\rim}{\mathbb{R}^{J\times K}}
\newcommand{\cx}{\set{C}}
\newcommand{\Rang}{{\rm Rang}}

\newcommand{\sign}{{\rm sign}}

%======================================================
% further abbreviations
%======================================================

% equations and arrays

\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bqt}{\begin{quote}}
\newcommand{\eqt}{\end{quote}}
\renewcommand{\span}[1]{{\rm span}\{ #1 \}}

% references and figures

\newcommand{\eqr}[1]{Eq.(\ref{#1})}
\newcommand{\figr}[1]{Figure \ref{#1}}

% arrows

\newcommand{\rar}{\rightarrow}
\newcommand{\Rar}{\Rightarrow}

%======================================================
% theorems SIAM style
%======================================================
%\newtheorem{theorem}{\sc Theorem}[section]
% \newtheorem{example}[theorem]{\sc Example}
% \newtheorem{propn}[theorem]{\sc Proposition}
% \newtheorem{ppty}[theorem]{\sc Property}
% \newtheorem{lemma}[theorem]{\sc Lemma}
% \newtheorem{eg}[theorem]{\sc Example}
% \newtheorem{definition}[theorem]{\sc Definition}
% \newtheorem{remark}[theorem]{\sc Remark}
% \newtheorem{cor}[theorem]{\sc Corollary}
% \newtheorem{notn}[theorem]{\sc Notation}
% \newtheorem{algm}[theorem]{\sc Algorithm}
% \newtheorem{code}[theorem]{\sc Code}
% \newtheorem{hyp}[theorem]{\sc Hypothesis}

%======================================================
% specials for Fourier analysis
%======================================================
\newcommand{\nxl}{\frac{n\pi x}{l}}
\newcommand{\mxl}{\frac{m\pi x}{l}}
\newcommand{\intl}{\int_{-l}^{l}}
\newcommand{\sumnN}{\sum_{n=1}^{N}}
\newcommand{\intab}{\int_a^b} 
\newcommand{\intpi}{\int_{-\pi}^{\pi}} 
%\newcommand{\qed}{\hfill $\Box$} 

\newcommand{\FH}{{\bf A}_{FH}}
\newcommand{\SHN}{S_{W,N}^{(\mb{H})}}

%======================================================
% numbering of equations
%======================================================
% equation numbers should be sectionnumber.equationnumber
%\numberwithin{equation}{section}

